The Incredible Shrinking Neural Network: New Perspectives on Learning Representations Through The Lens of Pruning

How much can pruning algorithms teach us about the fundamentals of learning representations in neural networks? And how much can these fundamentals help while devising new pruning techniques? A lot, it turns out. Neural network pruning has become a topic of great interest in recent years, and many different techniques have been proposed to address this problem. The decision of what to prune and when to prune necessarily forces us to confront our assumptions about how neural networks actually learn to represent patterns in data. In this work, we set out to test several long-held hypotheses about neural network learning representations, approaches to pruning and the relevance of one in the context of the other. To accomplish this, we argue in favor of pruning whole neurons as opposed to the traditional method of pruning weights from optimally trained networks. We first review the historical literature, point out some common assumptions it makes, and propose methods to demonstrate the inherent flaws in these assumptions. We then propose our novel approach to pruning and set about analyzing the quality of the decisions it makes. Our analysis led us to question the validity of many widely-held assumptions behind pruning algorithms and the trade-offs we often make in the interest of reducing computational complexity. We discovered that there is a straightforward way, however expensive, to serially prune 40-70% of the neurons in a trained network with minimal effect on the learning representation and without any re-training. It is to be noted here that the motivation behind this work is not to propose an algorithm that would outperform all existing methods, but to shed light on what some inherent flaws in these methods can teach us about learning representations and how this can lead us to superior pruning techniques.

==> extra_stuff.tex <==
---------------------------------------------------------
REASONS FOR NEURONS vs WEIGHTS:

1. Mozer Smolenskey's learning: Only few neurons are actually important, hence removing the useless ones makes sense.
2. Bhiksha's reason
3. When you remove or quantize weights you assume that the neurons similar weights emanate from are the same essentially. - explanation I gave to Brian - follows up on 1.
3. Removing Neurons vs weights obviously frees up more space.

One reason to choose to rank and prune individual neurons as opposed to weights is that there are far fewer elements to consider. Furthermore, the removal of a single weight from a large network is a drop in the bucket in terms of reducing a network's core memory footprint. If we want to reduce the \textit{size} of a network as efficiently as possible, we argue that pruning neurons instead of weights is more efficient computationally as well as practically in terms of quickly reaching a hypothetical target reduction in memory consumption. This approach also offers downstream applications a realistic expectation of the minimal increase in error resulting from the removal of a specified percentage of neurons. Such trade-offs are unavoidable, but performance impacts can be limited if a principled approach is used to find the best candidate neurons for removal. 

------------------------------------------------------------------------
Assumption about what happens inside the useless neurons before the non-reranking experiments:

What actually happens is that a few, elite neurons learn an approximation of the input-output function, and the remaining units must learn a complex interdependence function which cancels out their respective influence on the network output. Furthermore, assuming enough units exist to learn the function in question, increasing the number of parameters does not increase the richness or robustness of the learned approximation, but rather simply increases the likelihood of overfitting and the number of noisy parameters to be canceled during training. This is evinced by the fact that in many cases, multiple neurons can be removed from a network with no re-training and with negligible impact on the quality of the output approximation. In other words, there are few bipartisan units in a trained network. A unit is typically either part of the (possibly overfit) input-output function approximation, or it is part of an elaborate noise cancellation task force. Assuming this is the case, most of the compute-time spent training a neural network is likely occupied by this arguably wasteful procedure of silencing superfluous parameters, and pruning can be viewed as a necessary procedure to ``trim the fat.''

Conclusion AFTER the above mentioned experiments:

it is not as simple as a one-to-one mapping. The relevant and non-relevant neurons have some dependencies, you can't just remove non-relevant neurons from a network and expect no impact on the performance of the relevant once, hence you either need to re-evaluate the impacts (i.e rerank) or you can try retraining after every prune, which would kind of defeat the purpose of pruning, since it needs a 'fully-trained network'. Also, Since we wish to avoid retraining in order to stay consistent with most pruning algos out there (you can't compare apples to oranges), we go for the first alternative ---- more discussion below also


ALSO INCLUDE THIS ----> 
It is well known that too many free parameters in a neural network can lead to overfitting. Regardless of the number of weights used in a given network, as \cite{segee1991fault} assert, the representation of a learned function approximation is almost never evenly distributed over the hidden units, and thus the removal of any single hidden unit at random can actually result in a network fault. 

--------------------------------------------------------------
TO RETRAIN OR NOT TO RETRAIN:

We observed copious evidence of this phenomenon in our experiments, and this is the motivation behind our decision to evaluate the pruning algorithms in this study on the simple criteria of their ability to trim neurons \textit{without} any re-training. If we were to employ re-training as part of our evaluation criteria, we would arguably \textit{not} be evaluating the quality of our algorithm's pruning decisions per se but rather the ability of back-propagation trained networks to recover from faults caused by non-ideal pruning decisions, as suggested by the conclusions of \cite{segee1991fault} and \cite{mozer1989skeletonization}. Moreover, as \cite{fahlman1989cascade} discuss, due to the ``herd effect'' and ``moving target'' phenomena in back-propagation learning, the remaining units in a network will simply shift course to account for whatever error signal is re-introduced as a result of a bad pruning decision or network fault. So long as there are enough critical parameters to learn the function in question, a network can typically recover faults with additional training. This limits the conclusions we can draw about the quality of our pruning criteria when we employ re-training. 

In terms of removing units without re-training, what we discovered is that predicting the behavior of a network when a unit is to be pruned is very difficult, and most of the approximation techniques put forth in existing pruning algorithms do not fare well at all when compared to a brute-force search. To begin our discussion of how we arrived at our algorithm and set up our experiments, we review of the existing literature.

------------------------------------------------------------
REST OF INTRO:


\subsection{Pruning Techniques}

If we wanted to continually shrink a neural network down to minimum size, the most straightforward brute-force way to do it is to individually switch each element off and measure the increase in total error on the training set. We then pick the element which has the least impact on the total error, and remove it. Rinse and repeat. This is extremely computationally expensive, given a reasonably large neural network and training set. Alternatively, we might accomplish this using any number of much faster off-the-shelf pruning algorithms, such as Skeletonization (\cite{mozer1989skeletonization}), Optimal Brain Damage (\cite{lecun1989optimal}), or later variants such as Optimal Brain Surgeon \cite{hassibi1993second}. In fact, we borrow much of our inspiration from these algorithms, with one major variation: Instead of pruning individual weights, we prune entire neurons, thereby eliminating all of their incoming and outgoing weight parameters in one go, resulting in more memory saved, faster.

The algorithm developed for this paper is targeted at reducing the total number of neurons in a trained network, which is one way of reducing its computational memory footprint. This is often a desirable criteria to minimize in the case of resource-constrained or embedded devices, and also allows us to probe the limitations of pruning down to the very last essential network elements. In terms of generalization as well, we can measure the error of the network on the test set as each element is sequentially removed from the network. With an oracle pruning algorithm, what we expect to observe is that the output of the network remains stable as the first few superfluous neurons are removed, and as we start to bite into the more crucial members of the function approximation, the error should start to rise dramatically. In this paper, the brute-force approach described at the beginning of this section serves as a proxy for an oracle pruning algorithm. 





\cite{mozer1989using} argue that only a subset of the hidden units in a neural network actually latch on to the invariant or generalizing properties of the training inputs, and the rest learn to either mutually cancel each other's influence or begin overfitting to the noise in the data. -------------> SECOND PART OF THIS STATEMENT WAS NOT IN THE ORIGINAL PAPER. THEY NEVER TALKED ABOUT WHAT USELESS NEURONS DO

We leverage this idea in the current work to rank all neurons in pre-trained networks based on their effective contributions to the overall performance. We then remove the unnecessary neurons to reduce the network's footprint. Through our experiments we not only concretely validate the theory put forth by \cite{mozer1989using} but we also successfully build on  it to prune networks to 40 to 60 \% of their original size without any major loss in performance.


---------------------------------------------------------------
CONCLUSION:
\section{Conclusions \& Future Work}
In conclusion, we must first re-assert that we do not present this work as a bench-marking study of the algorithm we derived and tested. We have merely used this algorithm as a jumping off point to investigate the nature of learning representations in neural networks. What we discovered is that first and second order methods do not make particularly good pruning decisions, and can get hopelessly lost after making a bad pruning decision resulting in a network fault. Furthermore, the brute-force algorithm does surprisingly well, despite being computationally expensive. This method does \textit{so} well in fact, we argue that further investigation is warranted to make this algorithm computationally tractable, though we do not speculate on how that should be done here. 

We also observed strong evidence for the hypotheses of \cite{mozer1989skeletonization} regarding the ``dualist'' nature of hidden units, i.e. that learning representations are divided between units which either participate in the output approximation or learn to cancel each others influence. This suggests that neural networks may in fact learn a minimal network implicitly, though we cannot say for sure that this is the case without further investigation. A necessary experiment to this end would be to compare the size of network constructed using cascade correlation (\cite{fahlman1989cascade}) and compare it to the results described herein. 

We have presented a novel algorithm for pruning whole neurons from a trained neural network using a second-order Taylor series approximation of the change in error resulting from the removal a given neuron as a pruning criteria. We compared this method to a first order method and a brute-force serial removal method which exhaustively found the next best single neuron to remove at each stage. Our algorithm relies on a combination of assumptions similar to the ones made by \cite{mozer1989skeletonization} and \cite{lecun1989optimal} in the formulation of the Skeletonization and Optimal Brain Damage algorithms. 

First, we assumed that the error function with respect to each individual neuron can be approximated with a straight line or more precisely with a parabola. Second, for second derivative terms we consider only the diagonal elements of the Hessian matrix, i.e. we assume that each neuron-weight connection can be treated independently of the other elements in the network. Third, we assumed that pruning could be done in a serial fashion in which we find the single least productive element in the network, remove it, and move on. We found that all of these assumptions are deeply flawed in the sense that the true relevance of a neuron can only be partially approximated by a first or second order method, and only at certain stages of the pruning process. 

For most problems, these methods can usually remove between 10-30\% of the neurons in a trained network, but beyond this point their reliability breaks down. For certain problems, none of the described methods seem to perform very well, though for obvious reasons the brute-force method always exhibits the best results. The reason for this is that the error function with respect to each hidden unit is more complex than a simple second-order Taylor series can approximate. Furthermore, we have not directly taken into account the interdependence of elements within a network, though the work of \cite{hassibi1993second} could provide some guidance in this regard. This is another critical issue to investigate in the future. 

Re-training may help in this regard. We freely admit that our algorithm does not use re-training to recover from errors made in pruning decisions. We argue that evaluating a network pruning algorithm using re-training does not allow us to make fair comparisons between the kinds of decisions made by these algorithms. Neural networks are very good at recovering from the removal of individual elements with re-training and so this compensates for sub-optimal pruning criteria. 

We have observed that pruning whole neurons from an optimally trained network without major loss in performance is not only possible but also enables compressing networks to 40-70\% of their original size, which is of great importance in constrained memory environments like embedded devices. We cite the results of our experiments using the brute force criterion as evidence of this conclusion. However expensive, it would be extremely easy to parallelize this method, or potentially approximate it using a subset of the training data to decide which neurons to prune. This avoids the problem of trying to approximate the importance of a unit and potentially making a mistake. 

It would also be interesting to see how these methods perform on deeper networks and on some other popular and real world datasets. In our case, on the MNIST dataset, we observed that it was more difficult to prune neurons from a deeper network than from one with a single layer. We should expect this trend to continue as networks get deeper and deeper, which also calls into further question the reliability of the described first and second order methods. We did investigate the order in which neurons were plucked from each layer of the networks and we found that the brute force method primarily removes neurons from the deepest layer of the network first, but there was no obvious pattern in layer preference for the other two methods. 

Our experiments using the visualization of error surfaces and pruning decisions concretely establish the fact that not all neurons in a network contribute to its performance in the same way, and the observed complexity of these functions demonstrates limitations of the approximations we used. 

Finally, we encourage the readers of this work to take these results into consideration when making decisions as to which methods to use to improve network generalization or compress their models. It should be remembered that various heuristics may perform well in practice for reasons which are in fact orthogonal to the accepted justifications given by their proponents. 




==> less_math_error_approximation.tex <==
\subsubsection{Linear Approximation Approach}
We can use equation \ref{eq:ts3} to get the linear error approximation of the change in error due to the $k$th neuron being turned off and represent it as $\Delta E_{k}^1$ as follows:

\begin{align}
\Delta E_{k}^1 = - O_k\cdot \left.\pdv{E}{O}\right|_{O_k}
\end{align}

The derivative term above is the first-order gradient which represents the change in error with respect to the output a given neuron. This term can be collected during back-propagation. As we shall see further in this section, linear approximations are not reliable indicators of change in error but they provide us with an interesting basis for comparison with the other methods discussed in this paper.

\subsubsection{Quadratic Approximation Approach}
As above, we can use equation \ref{eq:ts3} to get the quadratic error approximation of the change in error due to the $k$th neuron being turned off and represent it as $\Delta E_{k}^2$ as follows:

\begin{align}
\Delta E_{k}^2 =  - O_k\cdot \left.\pdv{E}{O}\right|_{O_k} + 0.5\cdot O_k^2\cdot \left.\pdv[2]{E}{O}\right|_{O_k}
\end{align}

The additional second-order gradient term appearing above represents the quadratic change in error with respect to the output of a given neuron. This term can be generated by performing back-propagation using second order derivatives. Collecting these quadratic gradients involves some non-trivial mathematics, the entire step-by-step derivation procedure of which is provided in the Supplementary Material as an Appendix.

==> pruning_algorithm.tex <==
\subsection{Proposed Pruning Algorithm}
\begin{figure}
  \includegraphics[width=\linewidth]{intuition.pdf}
  \caption{The intuition behind 1st \& 2nd order neuron pruning decisions}
  \label{fig:intuition}
\end{figure}

Figure \ref{fig:intuition} shows a random error function plotted against the output of any given neuron. Note that this figure is for illustration purposes only. The error function is minimized at a particular value of the neuron output as can be seen in the figure. The process of training a neural network is essentially the process of finding these minimizing output values for all the neurons in the network. Pruning this particular neuron (which translates to getting a zero output from it will result in a change in the total overall error. This change in error is represented by distance between the original minimum error (shown by the dashed line) and the top red arrow. This neuron is clearly a bad candidate for removal since removing it will result in a huge error increase. 

The straight red line in the figure represents the first-order approximation of the error using Taylor Series as described before while the parabola represents a second-order approximation. It can be clearly seen that the second-order approximation is a much better estimate of the change in error.

One thing to note here is that it is possible in some cases that there is some thresholding required when trying to approximate the error using the 2nd order Taylor Series expansion. These cases might arise when the parabolic approximation undergoes a steep slope change. To take into account such cases, mean and median thresholding were employed, where any change above a certain threshold was assigned a mean or median value respectively.

Two pruning algorithms are proposed here. They are different in the way the neurons are ranked but both of them use $\Delta E_{k}$, the approximation of the change in error as the basis for the ranking. $\Delta E_{k}$ can be calculated using the Brute Force method, or one of the two Taylor Series approximations discussed previously.

The first step in both the algorithms is to  decide a stopping criterion. This can vary depending on the application but some intuitive stopping criteria can be: maximum number of neurons to remove, percentage scaling needed, maximum allowable accuracy drop etc. 

\subsubsection{Algorithm I: Single Overall Ranking}
The complete algorithm is shown in Algorithm \ref{algo1}. The idea here is to generate a single ranked list based on the values of $\Delta E_{k}$. This involves a single pass of second-order back-propagation (without weight updates) to collect the gradients for each neuron. The neurons from this rank-list (with the lowest values of $\Delta E_{k}$) are then pruned according to the stopping criterion decided. We note here that this algorithm is intentionally naive and is used for comparison only. 

\begin{algorithm}
 \caption{Single Overall Ranking}
 \label{algo1}
 \begin{algorithmic}
 \STATE{\textbf{Data:} An optimally trained network, training dataset}
 \STATE {\textbf{Output:}A pruned network}
 \STATE Initialize and define stopping criterion;
 
 \STATE Perform forward propagation over the training set;
 
  \STATE Perform second-order back-propagation without updating weights and collect linear and quadratic gradients;
  
  \STATE Rank the remaining neurons based on $\Delta E_{k}$;
  
 \WHILE{stopping criterion is not met}
 \STATE Remove the last ranked neuron;
  
  \ENDWHILE
\end{algorithmic}
\end{algorithm}
 
\subsubsection{Algorithm II: Iterative Re-Ranking}

In this greedy variation of the algorithm (Algorithm \ref{algo2}), after each neuron removal, the remaining network undergoes a single forward and backward pass of second-order back-propagation (without weight updates) and the rank list is formed again. Hence, each removal involves a new pass through the network. This method is computationally more expensive but takes into account the dependencies the neurons might have on one another which would lead to a change in error contribution every time a dependent neuron is removed. 

\begin{algorithm}
\caption{Iterative Re-Ranking}
 \label{algo2}
 \begin{algorithmic}
\STATE{\textbf{Data:} An optimally trained network, training dataset}
 \STATE {\textbf{Output:}A pruned network}
 \STATE Initialize and define stopping criterion;
 
 \WHILE{stopping criterion is not met}
  \STATE Perform forward propagation over the training set;
  
  \STATE Perform second-order back-propagation without updating weights and collect linear and quadratic gradients;
  
  \STATE Rank the remaining neurons based on $\Delta E_{k}$;
  
  
  \STATE Remove the worst neuron based on the ranking;
  
 \ENDWHILE
 
\end{algorithmic}
\end{algorithm}


==> retrain_vs_noretrain.tex <==
\subsection{To Retrain or not to Retrain}



==> taylor_series.tex <==
\subsection{Taylor Series Representation of Error}
Let us denote the total error from the optimally trained neural network for any given validation dataset by $E$. $E$ can be seen as a function of $O$, where $O$ is the output of any general neuron in the network. This error can be approximated at a particular neuron's output (say $O_k$) by using the 2nd order Taylor Series as,

\begin{align}
\hat E(O) \approx E(O_k) + (O-O_k)\cdot \left.\pdv{E}{O}\right|_{O_k} +  0.5\cdot (O-O_k)^2\cdot \left.\pdv[2]{E}{O}\right|_{O_k}\label{eq:ts1},
\end{align}


When a neuron is pruned, its output $O$ becomes 0. %From equation \ref{eq:ts1}, the contribution $E(0)$ of this neuron, then becomes:

%\begin{align}
%\hat E(0) \approx E(O_k) - O_k\cdot \left.\pdv{E}{O}\right|_{O_k} +  0.5\cdot O_k^2\cdot \left.\pdv[2]{E}{O}\right|_{O_k}\label{eq:ts2}
%\end{align}

Replacing $O$ by $O_k$ in equation \ref{eq:ts1} shows us that the error is approximated perfectly by equation \ref{eq:ts1} at $O_k$. So:%Using this and equation \ref{eq:ts2} we get:

\begin{align}
\Delta E_k = \hat E(0) - \hat E(O_k)= - O_k\cdot \left.\pdv{E}{O}\right|_{O_k} + 0.5\cdot O_k^2\cdot \left.\pdv[2]{E}{O}\right|_{O_k}\label{eq:ts3},
\end{align}

where $\Delta E_k$ is the change in the total error of the network when exactly one neuron ($k$) is turned off. Most of the terms in this equation are fairly easy to compute, as we have $O_k$ already from the activations of the hidden units and we already compute $\pdv{E}{O}|_{O_k}$ for each training instance during backpropagation. The $\small{\pdv[2]{E}{O}|_{O_k}}$ terms are a little more difficult to compute. This is derived in the appendix and summarized in the sections below. 


